Active Exploration in Markov Decision Processes

We introduce the active exploration problem in Markov decision processes (MDPs). Each state of the MDP is characterized by a random value and the learner should gather samples to estimate the mean value of each state as accurately as possible. Similarly to active exploration in multi-armed bandit (MAB), states may have different levels of noise, so that the higher the noise, the more samples are needed. As the noise level is initially unknown, we need to trade off the exploration of the environment to estimate the noise and the exploitation of these estimates to compute a policy maximizing the accuracy of the mean predictions. We introduce a novel learning algorithm to solve this problem showing that active exploration in MDPs may be significantly more difficult than in MAB. We also derive a heuristic procedure to mitigate the negative effect of slowly mixing policies. Finally, we validate our findings on simple numerical simulations.

==> app_mixing_issue.tex <==
\section{The Mixing Issue: A 3-state Example}\label{app:three.state}

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[thick,scale=0.9]
	\begin{scope}[every node/.style={circle,thick,draw}]
	\node (1) at (0,0) {$\sigma_1^2 = 1$};
	\node (2) at (2,0) {$\sigma_2^2 \ll 1$};
	\node (3) at (4,0) {$\sigma_3^2 = 1$};
	\end{scope}
	\begin{scope}[>={Stealth[black]},
	every node/.style={fill=white,circle},
	every edge/.style={draw=gray, thick},
	every loop/.style={draw=gray, thick, min distance=5mm,looseness=5}]
	\path[]
	(1) [->,thick] edge[in=200,out=150, loop left,thick] node[left] {$a_1$} (1)
	(3) [->,thick] edge[in=200,out=150, loop right,thick] node[right] {$a_2$} (3)
	(1) [->,thick] edge[bend right=30] node[below] {$a_2$} (2)
	(1) [<-,thick] edge[bend left=30] node[above] {$a_1$} (2)
	(2) [->,thick] edge[bend right=30] node[below] {$a_2$} (3)
	(2) [<-,thick] edge[bend left=30] node[above] {$a_1$} (3);  
	\end{scope}
	\end{tikzpicture}
	%\vspace{-0.3in}
	\caption{Deterministic 3-state 2-action MDP with $\sigma^2_1 \!=\! \sigma^2_3 \!=\! 1$ and $\sigma^2_2 \ll 1$ (set to 0.001 in Fig.~\ref{plot_mixing_3state}).}
	\label{fig:toy_MDP}
		%\vspace{-0.2in}
\end{figure}

When the budget $n$ is small, the solution of the problem~\eqref{eq:opt.function.asymptotic.lambda} may be very inefficient compared to the performance of the optimal finite-time policy. As an illustrative example, consider the MDP in Fig.~\ref{fig:toy_MDP}. In the ''unconstrained'' version of the problem, where states can be directly sampled, (i.e., the bandit setting), the optimal continuous allocation for  problem~\eqref{eq:opt.function.simplified} tends to $(0.5,0,0.5)$ as $\sigma^2(s_2)$ tends to 0. As soon as we introduce the constraint of the MDP structure, such allocation may not be realizable by any policy. In this MDP, solving problem~\eqref{eq:opt.function.asymptotic.lambda} returns a policy that executes the self-loop actions in $s_1$ and $s_3$ with high probability (thus moving to $s_2$ with low probability) and takes a uniformly random action in $s_2$. The resulting asymptotic performance does indeed approach the optimal unconstrained allocation, as the stationary distribution of the policy $(\eta(s_1), \eta(s_2),\eta(s_3))$ tends to $(0.5,0,0.5)$ for any arbitrary initial state $\overline{s}$. However for any finite budget $n$, this policy performs very poor since the agent would get stuck in $s_1$ (or $s_3$ depending on the initial state) almost indefinitely, thus making the mean estimation of $s_3$ (or $s_1$) arbitrarily bad. As a result, the optimal asymptotic policy mixes arbitrarily slowly as $\sigma^2(s_2)$ tends to zero and its finite-time performance is then arbitrarily far from the optimal performance. 

